The Role of Explanation Styles and Perceived Accuracy on Decision Making in Predictive Process Monitoring

Predictive Process Monitoring (PPM) often uses deep learning models to predict the future behavior of ongoing processes, such as predicting process outcomes. While these models achieve high accuracy, their lack of interpretability undermines user trust and adoption. Explainable AI (XAI) aims to address this challenge by providing the reasoning behind the predictions. However, current evaluations of XAI in PPM focus primarily on functional metrics (such as fidelity), overlooking user-centered aspects such as their effect on task performance and decision-making. This study investigates the effects of explanation styles (feature importance, rule-based, and counterfactual) and perceived AI accuracy (low or high) on decision-making in PPM. We conducted a decision-making experiment, where users were presented with the AI predictions, perceived accuracy levels, and explanations of different styles. Users' decisions were measured both before and after receiving explanations, allowing the assessment of objective metrics (Task Performance and Agreement) and subjective metrics (Decision Confidence). Our findings show that perceived accuracy and explanation style have a significant effect.

==> Body/52statistictests.tex <==

The variables used for testing the hypotheses varied depending on the specific hypothesis. Table \ref{tab:stat} outlines the variables and statistical methods employed for each hypothesis. For all tests, we used G*Power to calculate the required sample size based on a mid-effect size to ensure valid results.

Hypotheses H1, H4, and H7, which examine the influence of AI accuracy, were tested using Independent Samples T-Tests. For these tests, G*Power calculations indicated that 88 participants were needed per accuracy group (high and low) with the following parameters: effect size = 0.5, $\alpha$ = 0.05, and power (1-$\beta$ err prob) = 0.95. Although one participant was missing from the high-accuracy group, we excluded them to maintain data quality.

Hypotheses H2, H5, and H8, which focus on outcomes after explanations are provided, were analyzed using One-Way ANOVA followed by Tukey HSD post-hoc tests. G*Power calculations with an effect size = 0.25, $\alpha$ = 0.05, and power (1-$\beta$ err prob) = 0.8 indicated that 26 participants were needed per explanation style group across both high and low accuracy, totalling 156 participants. For these hypotheses, we recruited sufficient participants for testing.

Hypotheses H3, H6, and H9, which assess changes before and after explanations, were tested using Paired Samples T-Tests. For these tests, G*Power calculations (effect size d = 0.5, $\alpha$ = 0.05, power (1-$\beta$ err prob) = 0.80) indicated that 26 participants per group were sufficient.

Apart from H1, H4, and H7, the remaining hypotheses were also analyzed separately for the high-accuracy and low-accuracy groups to explore the differential effects of perceived AI accuracy. Additionally, we conducted analyses combining explanation styles regardless of accuracy levels.

\begin{table}[H]
\renewcommand{\arraystretch}{2}
\caption{Analytical Approaches per Hypotheses}
\label{tab:stat}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
\hline
\textbf{Measure Task} & \textbf{Hypotheses} & \textbf{IV} & \textbf{DV} & \textbf{Analysis Method} \\ \hline
\multirow{3}{*}{Task Performance (TP)} & H1 & Perceived AI Acc. & Initial TP & Independent t-test \\
 & H2 & Exp. styles & Post TP & One-way ANOVA \\
 & H3 & Exp. styles & Initial TP - Post TP & Paired t-test \\
 &  &  &  &  \\
Agreement (Agg.) & H4 & Perceived AI Acc. & Initial Agg. & Independent t-test \\
 & H5 & Exp. styles & Post Agg. & One-way ANOVA \\
 & H6 & Exp. styles & Initial Agg.-Post Agg. & Paired t-test \\
 &  &  &  &  \\
Decision Confidence (DC) & H7 & Perceived AI Acc. & Initial DC & Independent t-test \\
 & H8 & Exp. styles & Post DC & One-way ANOVA \\
 & H9 & Exp. styles & Initial DC - Post DC & Paired t-test \\ \hline
\end{tabular}%
}
\end{table}
